Transforming a Quadruped into a Guide Robot for the Visually Impaired: Formalizing Wayfinding, Interaction Modeling, and Safety Mechanism

This paper explores the principles for transforming a quadrupedal robot into a guide robot for individuals with visual impairments. A guide robot has great potential to resolve the limited availability of guide animals that are accessible to only two to three percent of the potential blind or visually impaired (BVI) users. To build a successful guide robot, our paper explores three key topics: (1) formalizing the navigation mechanism of a guide dog and a human, (2) developing a data-driven model of their interaction, and (3) improving user safety. First, we formalize the wayfinding task of the human-guide robot team using Markov Decision Processes based on the literature and interviews. Then we collect real human-robot interaction data from three visually impaired and six sighted people and develop an interaction model called the ``Delayed Harness'' to effectively simulate the navigation behaviors of the team. Additionally, we introduce an action shielding mechanism to enhance user safety by predicting and filtering out dangerous actions. We evaluate the developed interaction model and the safety mechanism in simulation, which greatly reduce the prediction errors and the number of collisions, respectively. We also demonstrate the integrated system on a quadrupedal robot with a rigid harness, by guiding users over $100+$~m trajectories.

==> manuscript/data/table-noise-collfree.tex <==

\begin{table}
\begin{center}
\begin{tabular}{@{}ccc|c@{}}
\toprule
\textbf{Sensor} & \textbf{Train Noise} & \textbf{Test Noise} & \textbf{Collision-Free Ep. Cnt} \\ \midrule
Depth & - & - & 8 \\
{Depth} & {-} & \checkmark & 5 \\
Depth & \checkmark & \checkmark & 12 \\
Depth + Lidar & \checkmark & \checkmark & \textbf{14} \\ \bottomrule
\end{tabular}
\end{center}
\caption{Collision-free episode count comparison to examine safety under noise using additional Lidar sensor}
\label{table:asym-noise}
\end{table}
% \begin{table}[]
% \begin{tabular}{cc|ccc}
% \hline
% Sensor Configuration & train action scale & Collision-free episode count & collision count & travel distance \\ \hline
% \multirow{5}{*}{Ideal} & 0 & - (diverge) & - (diverge) & - (diverge) \\
%  & 0.1 & \textbf{24} & \textbf{0.0} & 2.1 \\
%  & 0.5 & 21 & 1.5 & 3.4 \\
%  & 0.9 & 22 & 1.8 & 3.8 \\
%  & 1.0 (no shielding) & 23 & 1.4 & \textbf{6.1} \\ \hline
% \multirow{4}{*}{Aliengo} & 0 & 16 & 157.6 &  \\
%  & 0.1 & 17 & 4.12 &  \\
%  & 0.5 & \textbf{21} & \textbf{1.48} &  \\
%  & 1.0 (no shielding) & 18 & 3.16 & \multicolumn{1}{l}{} \\ \cline{2-5} 
% \end{tabular}
% \end{table}
